LUXOR: An FPGA Logic Cell Architecture for Efficient Compressor Tree Implementations

We propose two tiers of modifications to FPGA logic cell architecture to deliver a variety of performance and utilization benefits with only minor area overheads. In the irst tier, we augment existing commercial logic cell datapaths with a 6-input XOR gate in order to improve the expressiveness of each element, while maintaining backward compatibility. This new architecture is vendor-agnostic, and we refer to it as LUXOR. We also consider a secondary tier of vendor-speciic modifications to both Xilinx and Intel FPGAs, which we refer to as X-LUXOR+ and I-LUXOR+ respectively. We demonstrate that compressor tree synthesis using generalized parallel counters (GPCs) is further improved with the proposed modifications. Using both the Intel adaptive logic module and the Xilinx slice at the 65nm technology node for a comparative study, it is shown that the silicon area overhead is less than 0.5% for LUXOR and 5-6% for LUXOR+, while the delay increments are 1-6% and 3-9% respectively. We demonstrate that LUXOR can deliver an average reduction of 13-19% in logic utilization on micro-benchmarks from a variety of domains.BNN benchmarks benefit the most with an average reduction of 37-47% in logic utilization, which is due to the highly-efficient mapping of the XnorPopcount operation on our proposed LUXOR+ logic cells.

==> sections/06-discussions.tex <==
%!TEX root=../draft.tex

\section{Discussions}

\subsection{Limitations}

Modeling the FPGA logic elements is a difficult task, given the lack of
technical details in each FPGA vendor's technical documentation. Furthermore,
the standard cell library used for synthesis is unlikely to match the actual
speed grade of comparable FPGAs. Since the development of an ASIC involves a
multitude of optimization stages that extract the best area/delay performance,
we cannot say with certainty that the synthesis results reported in this work
are highly accurate for the baseline and proposed changes. Nevertheless, we
have tried to create both Xilinx and Intel logic primitives to our best
capability, and are confident that they present a ground truth that would scale
well with each subsequent process. We hope to continue improving on the design,
and also to release LUXOR under an open-source licence, alongside the developed
software tools, such that it promotes FPGA architecture design in the future.

\subsection{Future Work / Discussions}

Discuss other loose technical points? Perhaps share a roadmap for LUXOR.


==> sections/nn-Informations.tex <==
%!TEX root=../draft.tex

\section{Information}

% \cite{DBLP:conf/date/VermaI07} Although this paper is investigating large parallel counters, they mentioned that compressor trees are heavily XOR-dominated. Sine the ASIC synthesizers are poor in XOR-intensive circuits (in 2007), optimized implementation of counter is required. However, they targets ASIC and they show large counters (up to 7-input counters) implementations using "selective expression method" rather than old approaches, such as only FA/HA-based compressor trees.


{\bf Compressors vs. CPAs}
Compressors are look like carry propagate adders, since they have carry in and carry out signals. However, in practice they works like GPCs. as their carry signals can propagate to one or two adjacent unite and the propagation chain is short. In contrast in carry propagation adder, the carry chain is as long as number of FA in the adder and carry chain normally dictate the critical path (delay). 


ILP solver: 
\begin{itemize}
    \item Greedy vs. ILP: it is shown in many previous works that in general ILP methods produce better results in the cost of more run-time~\cite{DBLP:conf/date/VermaI07}. 
    \item Please report the range of run-times for our ILP solver.
    \item please mention the highest priority for our solver was less stage number rather than number of LUTs.
\end{itemize}
 
{\bf Sid, please note this point: in Intel architecture we have true and native support of ternary adder. How ever there is an implementation on Xilinx architecture to support ternary adder using general interconnection rather than carry-chain as proposed in \cite{ug384,DBLP:phd/dnb/Kumm16}.
%https://link.springer.com/content/pdf/10.1007%2F978-3-658-13323-8_10.pdf
This paper \cite{DBLP:conf/mbmv/KummZ14}  claims the performance of this implementation is equal to two layer of 2-input carry propagation adder and using that is non sense.}






why not adding MajFA into Xilinx? 
1) C25:121 already can implemented using 2LUTs
2) to improve it we should use 1 LUT
3) it requires 4 output 
4) each LUT provide 2-3 outputs 
So, it is impossible

Lets talk a line about FPCAs: which are homogeneous array of arithmetic primitives and a general interconnection network which can be used like DSP block for specific implementations. 




==> sections/unused.tex <==
\begin{table*}[t]
\renewcommand{\arraystretch}{1.3}
\caption{Comparison of Tomas paper and our ILP + reports of our modification's improvements using Tomas Compressor list}
\label{table_solver_xilinx}
\centering
%\multicolumn{4}{|c||}
%\multirow{2}{*}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
    \cline{2-15}
    \multicolumn{1}{c|}{} & \multicolumn{6}{c|}{Tomas Paper} & \multicolumn{8}{c|}{Our ILP}\\
    \hline
    {Input} & \multicolumn{3}{c|}{Heuristic Efficiency} & \multicolumn{3}{c|}{Heuristic Strength} & \multicolumn{2}{c|}{Tomas} & \multicolumn{3}{c|}{+XOR6} & \multicolumn{3}{c|}{+XOR6+Carry}\\
    \cline{2-15}
    {matrix} & {LUTs} & {stage} & {Total LUTs} & {LUTs} & {stage} & {Total LUTs} & {LUTs} & {stages} & {LUTs} & {stages} & {ratio} & {LUTs} & {stages} & {ratio}\\
    \hline
    {128} & {96} & {4} & {101} & {97} & {3} & {102} & {92} & {3} & {71} & {3} & {0.77} & {70} & {3} & {0.76} \\
    \hline
    {256} & {203} & {4} & {209} & {202} & {4} & {209} & {186} & {4} & {147} & {4} & {0.79} & {142} & {4} & {0.76} \\
    \hline
    {512} & {412} & {5} & {418} & {415} & {5} & {422} & {370} & {5} & {302} & {5} & {0.82} & {} & {} & {0} \\
    \hline
    {128,128} & {172} & {5} & {178} & {198} & {4} & {205} & {158} & {4} & {142} & {4} & {0.90} & {} & {} & {0} \\
    \hline
    {256,256} & {351} & {6} & {360} & {409} & {5} & {417} & {317} & {5} & {} & {} & {} & {} & {} & {} \\
    \hline
    {512,512} & {713} & {7} & {721} & {831} & {6} & {839} & {} & {} & {} & {} & {} & {} & {} & {} \\
    \hline
\end{tabular}
\end{table*}


\begin{table}
\renewcommand{\arraystretch}{1.3}
\caption{rough results of some synthesis (using our algorithm (Pulp ILP))}
\label{table_ILP}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
    \hline
    \multirow{2}{*}{Benchmark} & \multicolumn{2}{c|}{Cost (Stage / LUT)} & \multicolumn{2}{c|}{reduction} & {Run Time}\\
    \cline{2-5}
    {} & {baseline} & {+XOR6} & {LUT} & {\%} & {(s)}\\
    \hline
    {four 3-bit} & {2 / 4} & {2 / 4} & {0} & {0} & {0.1-0.2}\\
    \hline
    {eight 8-bit} & {3 / 31} & {3 / 29} & {2} & {6.5} & {27-48}\\
    \hline
    {Pop-256} & {5 / 227} & {5 / 162} & {65} & {28.6} & {2.5-2.7}\\
    \hline
    {Pop-1024} & {6 / 988} & {6 / 675} & {313} & {31.6} & {11-164}\\
    \hline
    %{} & {} & {} & {} & {} & {}\\
    %\hline
\end{tabular}
\end{table}


% \begin{table}[t]
% \renewcommand{\arraystretch}{1.3}
% \caption{Other benchmarks}
% \label{table_solver_xilinx}
% \centering
% \setlength{\tabcolsep}{2pt}
% %\multicolumn{4}{|c||}
% %\multirow{2}{*}
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
%     \hline
%     \multirow{3}{*}{Inputs} & \multicolumn{3}{c|}{Xilinx Architecture} & \multicolumn{4}{c|}{Intel Architecture}\\
%     \cline{2-8}
%     {} & \multirow{2}{*}{B} &\multirow{2}{*}{+XOR} & {+XOR} & \multirow{2}{*}{B} & \multirow{2}{*}{+XOR} & \multirow{2}{*}{+MFA} & {+XOR} \\
%     {} & {} & {} & {+Carry} & {} & {} & {} & {+MFA} \\
%     \hline 
%     {3-MAC 4$\times$4} & {} & {} & {} & {} & {} & {} & {} \\
%     \hline
%     {3-MAC 6$\times$6} & {} & {} & {} & {} & {} & {} & {} \\
%     \hline
%     {3-MAC 8$\times$8} & {} & {} & {} & {} & {} & {} & {} \\
%     \hline
%     {3-MAC 10$\times$10} & {} & {} & {} & {} & {} & {} & {} \\
%     \hline
%     {3-MAC 12$\times$12} & {} & {} & {} & {} & {} & {} & {} \\
%     \hline
%     {3-MAC 14$\times$14} & {} & {} & {} & {} & {} & {} & {} \\
%     \hline
%     {3-MAC 16$\times$16} & {} & {} & {} & {} & {} & {} & {} \\
%     \hline
%     {FIR-3} & {} & {} & {} & {} & {} & {} & {} \\
%     \hline
%     {4 4-bit adder} & {} & {} & {} & {} & {} & {} & {} \\
%     \hline
%     {6 6-bit adder} & {} & {} & {} & {} & {} & {} & {} \\
%     \hline
%     {8 8-bit adder} & {} & {} & {} & {} & {} & {} & {} \\
%     \hline
%     {12 12-bit adder} & {} & {} & {} & {} & {} & {} & {} \\
%     \hline
%     {14 14-bit adder} & {} & {} & {} & {} & {} & {} & {} \\
%     \hline
%     {16 16-bit adder} & {} & {} & {} & {} & {} & {} & {} \\
%     \hline
% 
% \end{tabular}
% \end{table}
% 

==> tables/comp_intel_full.tex <==
%!TEX root=../draft.tex

\begin{table}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.0}

\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\newcolumntype{L}[1]{>{\arraybackslash}m{#1}}

\caption{Comparison of different GPCs proposed in \cite{DBLP:journals/corr/abs-1806-08095} and new GPCs supported by LUXOR and LUXOR$+$}
\label{table_intel_GPCs}
\centering
\begin{tabular}{|c|l||c|c|c|c|c|c|c|c|}
% \begin{tabular}{|M{10mm}|L{10mm}||M{10mm}|M{10mm}|M{10mm}|M{10mm}|M{10mm}|M{10mm}|M{10mm}|M{10mm}|}
    %\multirow{2}{*}{}
    %\multicolumn{2}{c|}{}
    %\rotatebox{90}{old}
    \hline
    \multicolumn{2}{|c||}{\multirow{2}{*}{GPCs}} & \multirow{2}{*}{$S$} & \multirow{2}{*}{$A$} & \multicolumn{3}{c|}{LUT-based} & \multicolumn{3}{c|}{Arithmetic}\\
    \cline{5-10}
    \multicolumn{2}{|c||}{} & {} & {} & {Delay} & {LUTs} & {$APD$} & {Delay} & {LUTs} & {$APD$}\\
    \hline
    \hline
    \multirow{9}{*}{\cite{DBLP:journals/trets/Parandeh-AfsharNBI11}}&{C6:111} & {2} & {0.13} & {\bf 0.38} & {3}  & {\bf 7.9} & {0.97} & {2} & {4.6}\\
    \cline{2-10}
    {}&{C15:111} & {2} & {0} & {\bf 0.38} & {3} & {\bf 7.9} & {0.97} & {2} & {4.6}\\
    \cline{2-10}
    {}&{C23:111} & {1.67} & {0} & {\bf 0.38} & {2} & {\bf 5.3} & {0.97} & {2} & {2.1}\\
    \cline{2-10}
    {}&{C7:111} & {2.33} & {0} & {1.36} & {4} & {1.3} & {0.98} & {2.5} & {6.5}\\
    \cline{2-10}
    {}&{C16:1111} & {1.75} & {0.44} & {1.36} & {5} & {2.3} & {1.01} & {3} & {3}\\
    \cline{2-10}
    {}&{C35:1111} & {2} & {0.25} & {1.36} & {5} & {2.4} & {1.01} & {3} & {5.3}\\
    \cline{2-10}
    {}&{C44:1111} & {2} & {0.19} & {1.36} & {5} & {2.4} & {1.01} & {3} & {5.3}\\
    \cline{2-10}
    {}&{C53:1111} & {2} & {0.13} & {1.36} & {5} & {2.4} & {1.01} & {3} & {5.3}\\
    \cline{2-10}
    {}&{C62:1111} & {2} & {0.06} & {1.36} & {5} & {2.4} & {1.01} & {3} & {5.3}\\
    \hline
    \hline
    {\cite{DBLP:journals/corr/abs-1806-08095}}&{C25:121} & {1.75} & {0} & {0.38} & {\bf 2} & {\bf 11.8} & {-} & {-} & {-}\\
    \hline
    \hline
    \multirow{2}{*}{\rotatebox{90}{Ours}}&{C6:111} & {2} & {0.13} & {0.39*} & {2} & {\bf 10.95*} & {-} & {-} & {-}\\
    \cline{2-10}
    {}&{C25:121} & {1.75} & {0} & {0.39*} & {1} & {\bf 21.9*} & {-} & {-} & {-}\\
    \hline
    %\multirow{2}{*}{\rotatebox{90}{Ours}}&{C6:111} & {2} & {\bf 0.13} & {0.39*} & {\bf 2.1*} & {\bf 10.95} & {-} & {-} & {-}\\
    %\cline{2-10}
    %{}&{C25:121} & {1.75} & {\bf 0} & {0.39*} & {\bf 1.05*} & {\bf 21.9} & {-} & {-} & {-}\\
    %\hline
    
    \multicolumn{10}{L{85mm}}{\footnotesize \color{purple}*Calculated by scaling the reported delay of the baseline C6:111 GPC and the new LUT cost with the observed timing and area overhead of I-LUXOR+ from our synthesis experiments (respectively 3 and 5\%).}
   
\end{tabular}
\end{table}

==> tables/comp_summary.tex <==
\begin{table}
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{2.2pt}
\caption{{\color{purple} This Table can be removed} GPCs / Compressors used in this paper}  %\cite{DBLP:journals/corr/abs-1806-08095}}
\label{table_compressor_sets}
\centering
\begin{tabular}{|m{0.8em}|m{4.0em}|m{19.4em}|}
    %\multirow{2}{*}{}
    %\multicolumn{2}{c|}{}
    \cline{3-3}
    \multicolumn{2}{c|}{} & {\bf Name [Cost in LUTs]}\\
    \hline
    \multirow{3}{*}{\rotatebox{90}{\bf Xilinx}} & {\bf Baseline} & {
    \shortstack[l]{(C3:11) [1], (C$25\text{:}121$) [2], (C$6\text{:}111$) [3], (C1325:5)\\ {[4], All baseline combinations of Table~\ref{table_Xilinx_new_slice_based_compressor} [4]} %three Atoms:  \{-06-, -14-, and -22-\} [4]
    \\4-coupled ($4\text{:}2$) compressor [4]}}\\
    \cline{2-3}
    {} &  {\bf LUXOR} & {Baseline + (C$6\text{:}111$) [2]}\\
    \cline{2-3}
    {} &  {\bf LUXOR+}  & {LUXOR + combinations of Table~\ref{table_Xilinx_new_slice_based_compressor} [4]
    %All combinations of four atoms: \{-0606-, -06-, -14-, and -22-\} [4]
    }\\
    \hline
    \hline
    \multirow{3}{*}{\rotatebox{90}{\bf Intel}} & {\bf Baseline} & {(C3:11) [1], (C$25\text{:}121$) [2], (C$6\text{:}111$) [3], (C$15\text{:}111$) [2], (C$23\text{:}111$) [2]}\\
    \cline{2-3}
    {}&  {\bf LUXOR}  & {Baseline + (C$6\text{:}111$) [2]}\\
    \cline{2-3}
    {}&  {\bf LUXOR+}  & {I-LUXOR + (C$25\text{:}121$) [1]}\\
    \hline
\end{tabular}
\end{table}

%\begin{table}
%\renewcommand{\arraystretch}{1.3}
%\setlength{\tabcolsep}{2pt}
%\caption{GPCs / Compressors used in this paper  %\cite{DBLP:journals/corr/abs-1806-08095}}
%\label{table_compressor_sets}
%\centering
%\begin{tabular}{|m{0.8em}|m{9em}|m{14.5em}|}
    %\multirow{2}{*}{}
    %\multicolumn{2}{c|}{}
%    \cline{2-3}
%    \multicolumn{1}{c|}{} & {GPC/Compressor type} & {Name (cost)}\\
%    \hline
%    \multirow{4}{*}{\rotatebox{90}{\bf Xilinx}} & {LUT-based GPCs} & {FA(1), C6:111(3), and C25:121(2)}\\
%    \cline{2-3}
%    {} & {Slice-based GPCs} & {C1325:5(4), All combinations of three Atoms: -06-, -14-, and -22- (4)}\\
%    \cline{2-3}
%    {} & {Slice-based} & {4-coupled Compressor 4:2 (4)}\\
%    \hline
%    \hline
%    {\rotatebox{90}{\bf Intel}}& {LUT-based} & {C6:111 (3), C25:121 (2), C15:111 (2), FA (1), C23:111 (2)}\\
%    \hline
%\end{tabular}
%\end{table}




==> tables/synthesis.tex <==
%!TEX root=../draft.tex

\begin{table}
\renewcommand{\arraystretch}{1.3}
%\setlength{\tabcolsep}{4.5pt}
\caption{ASIC results of an ALM by adding 6-input XOR gate and Maj-3+FA circuits (individually and together)}
\label{table_ASIC}
\centering
\begin{tabular}{|c|c|c|c|c|}
    \hline
    \multicolumn{5}{|c|}{Timing optimized}\\
    \hline
    {Metrics} & {baseline} & {+XOR6} & {+Maj3+FA} & {+XOR6+Maj3+FA}\\
    \hline
    {Area} & {1680} & {1687} & {1715} & {1767}\\
    \hline
    {Delay} & {0.19} & {0.18} & {0.18} & {0.18}\\
    \hline
    {Area(ratio)} & {1} & {1.004} & {1.020} & {1.051}\\
    \hline
    {Delay(ratio)} & {1} & {1} & {1} & {1}\\
    \hline
    \multicolumn{5}{|c|}{Area optimized (Area$\times$delay is 1.17$\times$ worse than Timing opt)}\\
    \hline
    {Metrics} & {baseline} & {+XOR6} & {+Maj3+FA} & {+XOR6+Maj3+FA}\\
    \hline
    {Area} & {1511} & {1556} & {1581} & {1628}\\
    \hline
    {Delay} & {0.23} & {0.23} & {0.24} & {0.23}\\
    \hline
    {Area(ratio)} & {1} & {1.030} & {1.046} & {1.078}\\
    \hline
    {Delay(ratio)} & {1} & {1} & {1} & {1}\\
    \hline
\end{tabular}
\end{table}


